Cusp forms and parabolic cohomology classes for symmetric spaces of rank one

For any rank-one Riemannian symmetric space S of non-compact type and any discrete, cofinite, non-cocompact, torsion-free group $\Gamma$ of orientation-preserving Riemannian isometries on S, we develop a cohomological interpretation for the cusp forms of $\Gamma$. To that end, we identify certain $\Gamma$-submodules of smooth semi-analytic vectors in the spherical principal series representation with spectral parameter $\nu$ as well as certain subspaces of parabolic cohomology spaces of $\Gamma$ of degree dim S-1 with these $\Gamma$-submodules. We provide explicit isomorphisms between the spaces of cusp forms of spectral parameter $\nu$ and these specific cohomology subspaces. The isomorphisms from cusp forms to cohomology are given by an integral transform, and the explicit form of the inverse isomorphism takes advantage of a certain reproducing property of the integral transform. The result is uniform for all these symmetric spaces and does not rely on their classification.

==> ccro2-switches.tex <==
%%%% switches %%%%%%%%%%%%
\let\iflabels=\iffalse

\let\ifindexindication=\iffalse
\let\iftxfonts=\iftrue
\let\ifhyperref=\iftrue

\let\synctex=1


\makeatletter
\@ifundefined{iflabels}{}{%
\iflabels
\usepackage[notcite,notref]{showkeys}
\fi}

%%%% end of switches %%%%



\@ifundefined{iftxfonts}{\usepackage[varg]{txfonts}}{%
\iftxfonts
\usepackage[varg]{txfonts}
% gives nicer result when printing
\fi}




\@ifundefined{ifindex}{\let\ifindex=\iffalse}{}

\makeatother




%file name at bottom of pages
\iffalse
\makeatletter \@ifundefined{version}{\def\version{}}{}
\@ifundefined{flnm}{}{%
% file name on bottom of page
\def\@oddfoot{\rm{\footnotesize{File name
\tt\flnm\version.tex}\quad\today\hfil\thepage}}
\let\@evenfoot\@oddfoot \addtolength{\textheight}{-.4cm}
\addtolength{\footskip}{.4cm} }
\makeatother
\fi


%%%%%%%%%% hyperref %%%%%%%%%%%%%%%%%%%%%%5

\makeatletter \@ifundefined{ifhyperref}{\let\ifhyperref=\iffalse}{}
\makeatother



%%%%%%%%%%%%%%%%%

% insertion of experimental texts


\makeatletter
\@ifundefined{ifinsert}{\let\ifinsert=\iffalse}{}
\makeatother


\newcommand\insrt[3]% file name, label start, label end
{ \ifinsert\green \lijn \tocrgl{\green Inserted text\endgreen}{p \pageref{#2}--\pageref{#3}}
Text inserted from  the file \texttt{#1.tex} on pp~\pageref{#2}--\pageref{#3}
\lijn\endgreen
\input{#1}
\green \lijn end insertion of \texttt{#1.tex} \lijn\endgreen\fi%
}



